Power-generation enhancements and upstream flow properties of turbines in unsteady inflow conditions

Energy-harvesting systems in complex flow environments, such as floating offshore wind turbines, tidal turbines, and ground-fixed turbines in axial gusts, encounter unsteady streamwise flow conditions that affect their power generation and structural loads. In some cases, enhancements in time-averaged power generation above the steady-flow operating point are observed. To characterize these dynamics, a nonlinear dynamical model for the rotation rate and power extraction of a periodically surging turbine is derived and connected to two potential-flow representations of the induction zone upstream of the turbine. The model predictions for the time-averaged power extraction of the turbine and the upstream flow velocity and pressure are compared against data from experiments conducted with a surging-turbine apparatus in an open-circuit wind tunnel at a diameter-based Reynolds number of $Re_D = 6.3\times10^5$ and surge-velocity amplitudes of up to 24% of the wind speed. The combined modeling approach captures trends in both the time-averaged power extraction and the fluctuations in upstream flow quantities, while relying only on data from steady-flow measurements. The sensitivity of the observed increases in time-averaged power to steady-flow turbine characteristics is established, thus clarifying the conditions under which these enhancements are possible. Finally, the influence of unsteady fluid mechanics on time-averaged power extraction is explored analytically. The theoretical framework and experimental validation provide a cohesive modeling approach that can drive the design, control, and optimization of turbines in unsteady flow conditions, as well as inform the development of novel energy-harvesting systems that can leverage unsteady flows for large increases in power-generation capacities.

==> m99_unused.tex <==
%% SECTION 2 %%


\subsection{An induction model for a periodically surging turbine}

We seek a potential-flow model for the flow in the upstream induction zone of a horizontal-axis turbine surging in the streamwise direction. We model the turbine as a porous disc, rather than applying Biot-Savart integration on vortex models of the turbine wake, so as to obtain physically interpretable expressions that do not require integration in space or time. Our approach is congruous with that of \cite{steiros_drag_2018}, who extended the work of \cite{taylor_aerodynamics_1944} and \cite{koo_fluid_1973} to predict the drag on porous plates.



\subsection{Time-averaged power extraction by a periodically surging actuator disc}
We now seek to relate the flow conditions upstream of the surging porous disc to the power that may be extracted by the disc. Equation \ref{eqn:uModel} allows the flow velocity at the upstream side of the disc, $u(r=0,x\rightarrow {x_2}^-,t) \equiv u_2$, to be derived. For $U(t) = 0$, Equation \ref{eqn:uModel} gives $u_2/u_1 = 1-a$, and the aforementioned interpretation of $a$ as the induction factor from 1D axial momentum theory holds. For $U(t)\neq0$, we have
\begin{equation}
\frac{u_2}{u_1} = 1-a\left(1 - \frac{U(t)}{u_1}\right).
\label{eqn:u2}
\end{equation}

The time-varying nature of the flow velocity incident on the disc suggests that the steady-flow 1D axial-momentum analysis of \cite{betz_maximum_1920} may be revisited to obtain a theoretical prediction for the maximum time-averaged power extracted from a periodically surging actuator disc. We consider a radially symmetric control volume, shown in Figure \ref{fig:CV}, that is split across the face of the actuator disc into upstream and downstream regions. This discontinuous control volume is defined by four streamwise stations: station 1 is located far upstream where the flow is unaffected by the presence of the disc, station 2 is located on the upstream face of the disc, station 3 is located on the downstream face of the disc, and station 4 is located far downstream of the disc where the flow properties no longer change appreciably with streamwise distance. We assume the bounding surfaces of the control volumes follow the smallest streamtube that contains the surging disc, such that no flow exits from the sides. Furthermore, the flow-normal control surfaces at stations 2 and 3 move at the same velocity as the disc, $U(t)$, such that the volumes defined by the upstream and downstream control surfaces change with time. Finally, following Betz's approach, we assume that the flow properties do not vary in the radial direction, so that the flow is one-dimensional. Enforcing conservation of mass in this system yields $u_1 A_1 = u_2 \pi R^2 = u_4 A_4$, where $A_1$ and $A_4$ are the cross-sectional areas of the streamtube at its inlet and outlet. Similarly, applying conservation of momentum yields $u_2 = \frac{1}{2}\left(u_1+u_4\right)$, or equivalently, $u_4 = 2u_2-u_1$. Lastly, assuming steady flow and constant streamtube cross-sectional area across the disc gives $u_2 = u_3$, so that the flow velocity remains continuous across the disc. All of these velocities are inertial quantities, referenced to the static-observer frame shown in Figure \ref{fig:CV}.

The drag force on the disc is equal to the sum of the forces on the upstream and downstream control volumes, which can be obtained by invoking conservation of momentum:
\begin{equation}
\vec{F}_{cv} = \frac{\partial}{\partial t} \int_{cv} \rho \vec{u}_{cv} \,dV + \int_{cs} \rho \vec{u}_{flux} \left(\vec{u}_{rel} \cdot d\vec{A}\right),
\label{eqn:CoM}
\end{equation}
where $\vec{u}_{cv}$ is the flow velocity inside the control volume, $\vec{u}_{flux}$ is the flow velocity at the control surface in a fixed frame, and $\vec{u}_{rel}$ is the flow velocity through the control surface relative to the control surface itself. In the absence of external forces on the domain, $\vec{F}_{cv}$ is equivalent to the net pressure force on the control volume. We define the upstream and downstream control volumes to be sufficiently large so that we may treat $u_{cv}$ as constant, i.e.\ $u_{cv}\approx u_1$ for the upstream control volume and $u_{cv}\approx u_4$ for the downstream control volume. For a streamtube with a sufficiently small expansion angle at the disc, we may assume that the change in volume due to the moving control surface is approximately cylindrical, and thus $\frac{\partial V}{\partial t} \approx \pi R^2 \frac{d x_2}{dt} = \pi R^2 U(t)$. For both control volumes, at the disc we have $u_{flux} = u_2$. Similarly, $u_{rel}=u_2-U$ on the moving boundaries of both control volumes. Evaluating Equation \ref{eqn:CoM} with these quantities for each control volume and summing the results gives the drag force on the disc,
\begin{multline}
F_D = F_{cv,u} + F_{cv,d} = \rho\pi R^2 \left(u_1 U + u_2 (u_2 - U)\right) - \rho A_1 {u_1}^2 \\- \rho\pi R^2 \left(u_4 U + u_2 (u_2 - U)\right) + \rho A_4 {u_4}^2.
\label{eqn:thrust0}
\end{multline}
The thrust force is defined as the opposite of the drag force. After substituting for $A_1$, $A_4$, and $u_4$ in terms of $u_1$ and $u_2$, this can be written as
\begin{equation}
F_T = \rho\pi R^2 \left(- u_1 U + u_1 u_2 + u_4 U - u_2 u_4\right) = 2\rho\pi R^2 (u_1-u_2)(u_2-U).
\label{eqn:thrust}
\end{equation}
The instantaneous power extracted by the actuator disc can then be written as the product of the thrust force and the incident flow velocity relative to the disc at station 2,
\begin{equation}
\mathcal{P} = F_T \left(u_2-U\right) = 2\rho \pi R^2 \left(u_2-U\right)^2 \left(u_1 - u_2\right).
\label{eqn:pwrBetz}
\end{equation}
Substituting the definition of $u_2$ from Equation \ref{eqn:u2} and normalizing gives a simple expression for the instantaneous coefficient of power:
\begin{equation}
C_p(t) \equiv \frac{\mathcal{P}}{\frac{1}{2}\rho \pi R^2 {u_1}^3} = 4a(1-a)^2\left(1-\frac{U(t)}{u_1}\right)^3.
\label{eqn:Cp_t}
\end{equation}
When $U=0$, this expression simplifies to the Betz result, i.e.\ $C_{p,0} = 4a(1-a)^2$. To compute the time-averaged power extracted by the disc for a periodic surge-velocity waveform $U(t)$ with frequency $f$, we integrate Equation \ref{eqn:Cp_t} over a single surge period,
\begin{equation}
\overline{C_p} = \frac{f}{2\pi} \int_0^{\frac{2\pi}{f}} 4a(1-a)^2 \left(1 - \frac{U(t)}{u_1}\right)^3 dt,
\label{eqn:powerBetz}
\end{equation}
which for a sinusoidal surge-velocity waveform $U(t)/u_1 = u^* \sin(ft)$ integrates to
\begin{equation}
\frac{\overline{C_p}}{C_{p,0}} = 1 + \frac{3}{2} {u^*}^2.
\label{eqn:powerModel}
\end{equation}

The assumption of constant $C_p$ is analogous to the assumption of constant $a$ that is used in the present analysis, since according to the framework of Betz, $C_p$ is only dependent on $a$. It remains to be shown, however, that the problem of a surging turbine in uniform flow is equivalent to the problem of a stationary turbine in an oscillating inflow, at least within the assumptions of 1D axial momentum theory. It is to this consideration that we now turn our attention.

\subsection{On the problem of a stationary turbine in an oscillating inflow}

To model the power extracted from a stationary turbine in an oscillating inflow $u_1' = u_1 - U(t)$, we redefine the control volume shown in Figure \ref{fig:CV} so that the actuator disc is located at a fixed streamwise location and the upstream and downstream control volumes do not deform as a function of time. For a stationary disc, the potential-flow induction model in Equation \ref{eqn:uModel} gives $u_2' = u_1' (1-a)$. Assuming that the system behaves in a quasi-steady manner allows us to treat every instance of $u_1'(t)$ as an independent steady-flow problem, and thus these primed quantities may be substituted into the relations from steady-flow 1D axial momentum theory. Using conservation of mass and momentum, the instantaneous power extracted by the stationary disc can be written as
\begin{equation}
\mathcal{P} = 2\rho\pi R^2 {u_2'}^2 \left(u_1'-u_2'\right).
\label{eqn:powerStatDisc}
\end{equation}
Substituting for $u_1'$ and $u_2'$ and normalizing, we find that
\begin{equation}
C_p(t) = 4a(1-a)^2\left(1-\frac{U(t)}{u_1}\right)^3,
\label{eqn:Cp_t_statDisc}
\end{equation}
which is identical to the coefficient of power of a surging disc in uniform flow given in Equation \ref{eqn:Cp_t} above. This analysis shows that the expression for time-averaged power given by \cite{wen_influences_2017} and \cite{johlas_floating_2021} (Equation \ref{eqn:powerWenJohlas}) does indeed satisfy the conservation relations of 1D axial momentum theory. Moreover, we see that there is no difference between an oscillating turbine in uniform flow and a stationary turbine in an oscillatory inflow in terms of thrust force and power extraction -- given the assumptions of this quasi-steady analytical framework. In other words, within the present set of assumptions, the effects of turbine surge motions and inflow oscillations on turbine performance are identical. To reiterate, the key premise undergirding these conclusions is that $a$ remains constant with surge- or inflow-velocity amplitude. This premise will be interrogated empirically in the following sections.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Section 4: Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The fitted values of the induction factor $a$ across all experiments, shown in Figure \ref{fig:a_vs_u}, followed an increasing trend with surge-velocity amplitude $u^*$. A similar increasing trend was observed in the amplitude of the time-varying signal of the pressure difference between the upstream and downstream measurement locations, $p_{ud}(t)\equiv p(x=x_u,t)-p(x=x_d,t)$, which is plotted in Figure \ref{fig:dP}. In these plots, we denote amplitudes of fluctuations in time-varying quantities with a circumflex, e.g.\ $\hat{p}_{ud}$, to distinguish them from magnitudes of mean values. The fore-aft pressure difference can be understood as an analogue for turbine thrust, and in steady flow, higher thrust is associated with a larger velocity deficit upstream of the turbine and hence a higher induction factor. Therefore, we may qualitatively explain the increasing trend of the induction factor $a$ as a function of the surge-velocity amplitude $u^*$ as follows. If the thrust amplitude increases with $u^*$, as evidenced by the linearly increasing amplitude of the time-varying fluctuations of $p_{ud}$, then the amplitude of the time-varying flow-velocity fluctuations upstream of the turbine, $\hat{u}$, should increase as well. This is indeed observed in Figure \ref{fig:uHW_amp}. Equation \ref{eqn:PDT} shows that, for fixed surge kinematics $x_2(t)$ and $U(t)$, an increase in the amplitude of $u$ necessarily implies an increase in the induction factor $a$. Thus, we see that the increasing trend in $a$ as a function of $u^*$ shown in Figure \ref{fig:a_vs_u} is consistent with the increasing thrust amplitude suggested in Figure \ref{fig:dP}. Furthermore, integrating the expression for thrust given in Equation \ref{eqn:thrust} over a sinusoidal surge-velocity waveform, as done previously for $C_p(t)$, yields a time-averaged thrust enhancement of
\begin{equation}
\frac{\overline{F_T}}{F_{T,0}} = 1 + \frac{1}{2}{u^*}^2,
\label{eqn:thrustUnsteadyAvg}
\end{equation}
an increasing function with $u^*$. This increasing time-averaged thrust as a function of $u^*$ is also consistent with the trend between $a$ and $u^*$ shown in Figure \ref{fig:a_vs_u}, because, as previously discussed, higher mean-thrust states are associated with higher induction factors. We cannot directly confirm these arguments in the absence of thrust measurements, but they suggest that the behavior of $a$ is not unexpected within the present analytical framework.

To incorporate the dependence of $a$ on $u^*$ shown in Figure \ref{fig:a_vs_u} into the model, a linear fit was performed over all values of $a$, regardless of tip-speed ratio, and this fit for $a$ was used to compute models for the velocity and pressure for arbitrary surge-velocity amplitudes. These models, plotted in Figures \ref{fig:uHW_TF} and \ref{fig:p_TF}, demonstrated the same qualitative behavior as the measured data. The influence of tip-speed ratio was not modeled, so some deviations as a function of $\lambda$ that are not accounted for in the model trends are visible in the phase results. While the model is semi-empirical due to its reliance on the linear fit from Figure \ref{fig:a_vs_u}, the qualitative agreement in amplitude, phase, and waveform shape suggest that the assumptions undergirding the potential-flow model were reasonable within the upstream induction zone.

Finally, the time-averaged power measurements from these experiments were plotted against the surge-velocity amplitude $u^*$ in Figure \ref{fig:power} for the three tested tip-speed ratios. The data from the highest two tip-speed ratios increased with $u^*$, while the power produced at the lowest tip-speed ratio (near the optimal operating condition of the turbine) remained close to its steady value. As a reference, the model for time-averaged power given in Equation \ref{eqn:powerModel} was evaluated at $a=0.330=\langle a \rangle$, the average of the fitted induction factors from Figure \ref{fig:a_vs_u}. This was plotted as a dashed blue line in Figure \ref{fig:power}. The model captured the general trend of the data from the two higher tip-speed ratios, but overpredicted the power enhancements observed in the data at higher surge-velocity amplitudes. To account for the dependence of the induction factor $a$ on the surge-velocity amplitude $u^*$, the model for the time-averaged power was modified with a first-order expansion of $a$ about $a=\langle a \rangle$,
\begin{equation}
a\approx \langle a \rangle + \frac{\partial a}{\partial {u^*}} u^*,
\label{eqn:a_fit}
\end{equation}
where $\frac{\partial a}{\partial {u^*}} = 0.324$ is the slope of the linear fit shown in Figure \ref{fig:a_vs_u} above. The adjusted model, plotted as an orange dashed line in Figure \ref{fig:power}, showed closer agreement with the data. These results suggest that accounting for the dependence of turbine induction on surge velocity is important for capturing the time-averaged power production of periodically surging turbines.
